Playground v3: Improving Text-to-Image Alignment with Deep-Fusion Large Language Models

We introduce Playground v3 (PGv3), our latest text-to-image model that achieves state-of-the-art (SoTA) performance across multiple testing benchmarks, excels in graphic design abilities and introduces new capabilities. Unlike traditional text-to-image generative models that rely on pre-trained language models like T5 or CLIP text encoders, our approach fully integrates Large Language Models (LLMs) with a novel structure that leverages text conditions exclusively from a decoder-only LLM. Additionally, to enhance image captioning quality-we developed an in-house captioner, capable of generating captions with varying levels of detail, enriching the diversity of text structures. We also introduce a new benchmark CapsBench to evaluate detailed image captioning performance. Experimental results demonstrate that PGv3 excels in text prompt adherence, complex reasoning, and accurate text rendering. User preference studies indicate the super-human graphic design ability of our model for common design applications, such as stickers, posters, and logo designs. Furthermore, PGv3 introduces new capabilities, including precise RGB color control and robust multilingual understanding.

==> figs/mario-1k-movie.tex <==
\begin{figure*}
\includegraphics[width=1.0\textwidth]{images/gt-fluxpro-v3-0002.jpg}
\begin{tabular}{l}
    \multirow{6}{120mm}{\scriptsize{A romantic book cover featuring a couple in a close, affectionate pose. The woman, positioned on the left, has long, wavy brown hair and is wearing a sleeveless, patterned dress with a colorful beaded necklace. She is smiling softly and looking to her right. The man, positioned on the right, has short, dark hair and is wearing a gray suit jacket over a white shirt. He is smiling broadly and looking at the camera. The background is blurred with colorful bokeh lights, creating a vibrant and romantic atmosphere. The text 'His Unforgettable Fiancée' is written in white, bold, serif font in the bottom left corner, and 'Teresa Carpenter' is written in white, italic, serif font below it.}}
\end{tabular}
\vspace{18mm}

\caption{Qualitative comparison of text rendering accuracy in Mario-text-1k. From left to right: Ground Truth, Flux-pro and Playground V3.}

\label{fig:multiar-oct}
\end{figure*}
